Neural Natural Language Inference Models Partially Embed Theories of Lexical Entailment and Negation

We address whether neural models for Natural Language Inference (NLI) can learn the compositional interactions between lexical entailment and negation, using four methods: the behavioral evaluation methods of (1) challenge test sets and (2) systematic generalization tasks, and the structural evaluation methods of (3) probes and (4) interventions. To facilitate this holistic evaluation, we present Monotonicity NLI (MoNLI), a new naturalistic dataset focused on lexical entailment and negation. In our behavioral evaluations, we find that models trained on general-purpose NLI datasets fail systematically on MoNLI examples containing negation, but that MoNLI fine-tuning addresses this failure. In our structural evaluations, we look for evidence that our top-performing BERT-based model has learned to implement the monotonicity algorithm behind MoNLI. Probes yield evidence consistent with this conclusion, and our intervention experiments bolster this, showing that the causal dynamics of the model mirror the causal dynamics of this algorithm on subsets of MoNLI. This suggests that the BERT model at least partially embeds a theory of lexical entailment and negation at an algorithmic level.

==> interchange-schematic.tex <==
\newcommand{\repgap}{0.1cm}

\begin{tikzpicture}
  \tikzset{
    every node=[
    draw,
    font=\footnotesize,
    shape=rectangle,
    align=center,
    minimum width=0.6cm,
    minimum height=0.35cm,
    text width=0.6cm
    ],
    input/.style={
    },
    hiddenRed/.style={
      fill=red!30
    },
    hiddenBlue/.style={
      fill=blue!50
    },
    outputBlue/.style={
      trapezium,
      fill=blue!50,
      text=black,
      minimum height=0.5cm,
      minimum width=0.75cm
    },
    outputRed/.style={
      trapezium,
      fill=red!30,
      text=black,
      minimum height=0.5cm,
      minimum width=0.75cm
    },
    outputLabel/.style={
    },
    swap/.style={
      solid,
      thick,
      ->,
      shorten <=0pt,
      shorten >=0pt
    },
    replace/.style={
      dashed,
      thick,
      ->,
      shorten <=0pt,
      shorten >=0pt
    },
    ann/.style={
      minimum width=0.7cm,
      minimum height=0.5cm,
      text width=5cm,
      align=left,
    }   
};

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Network 1

  \node[input](x1){$x_{1}$};
  \node[input, right=\repgap of x1](x2){$x_{2}'$};
  \node[input, right=\repgap of x2](x3){$x_{3}'$};

  \node[hiddenBlue, above=\repgap of x1](h11){};
  \node[hiddenRed, right=\repgap of h11](h12){};
  \node[hiddenRed, right=\repgap of h12](h13){};

  \node[hiddenBlue, above=\repgap of h11](h21){};
  \node[hiddenBlue, right=\repgap of h21](h22){};
  \node[hiddenBlue, right=\repgap of h22](h23){};

  \node[hiddenBlue, above=\repgap of h21](h31){};
  \node[hiddenBlue, right=\repgap of h31](h32){};
  \node[hiddenBlue, right=\repgap of h32](h33){};

  \node[outputBlue, above=\repgap of h32](o1){$y$};
  %\node[outputLabel, above=0cm of o1](y1){$y$};

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Network 2

  \node[input, right=0.75cm of x3](xx1){$x_{1}$};
  \node[input, right=\repgap of xx1](xx2){$x_{2}$};
  \node[input, right=\repgap of xx2](xx3){$x_{3}$};

  \node[hiddenRed, above=\repgap of xx1](hh11){};
  \node[hiddenRed, right=\repgap of hh11](hh12){};
  \node[hiddenRed, right=\repgap of hh12](hh13){};

  \node[hiddenRed, above=\repgap of hh11](hh21){};
  \node[hiddenRed, right=\repgap of hh21](hh22){$L$};
  \node[hiddenRed, right=\repgap of hh22](hh23){};

  \node[hiddenRed, above=\repgap of hh21](hh31){};
  \node[hiddenRed, right=\repgap of hh31](hh32){};
  \node[hiddenRed, right=\repgap of hh32](hh33){};

  \node[outputRed, above=\repgap of hh32](o2){$z$};
  %\node[outputLabel, above=0cm of o2](y2){};


  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Network 3

  \node[input, below=2.4cm of x1](xxx1){$x_{1}$};
  \node[input, right=\repgap of xxx1](xxx2){$x_{2}$};
  \node[input, right=\repgap of xxx2](xxx3){$x_{3}$};

  \node[hiddenBlue, above=\repgap of xxx1](hhh11){};
  \node[hiddenBlue, right=\repgap of hhh11](hhh12){};
  \node[hiddenBlue, right=\repgap of hhh12](hhh13){};

  \node[hiddenBlue, above=\repgap of hhh11](hhh21){};
  \node[hiddenRed, right=\repgap of hhh21](hhh22){$L$};
  \node[hiddenBlue, right=\repgap of hhh22](hhh23){};

  \node[hiddenBlue, above=\repgap of hhh21](hhh31){};
  \node[hiddenBlue, right=\repgap of hhh31](hhh32){};
  \node[hiddenBlue, right=\repgap of hhh32](hhh33){};

  \node[outputBlue, above=\repgap of hhh32](o3){$y$};
  %\node[outputLabel, above=0cm of o3](y3){$y$};


  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Arrows

  \path(xx2.south) edge[swap, bend left=10pt] (x2.south);
  \path(xx3.south) edge[swap, bend left=10pt] (x3.south);

  \path(hh22.south) edge[replace, bend left=10pt] (hhh22.east);

\end{tikzpicture}
